Towards a Health-Based Power Grid Optimization in the Artificial Intelligence Era

The electric power sector is one of the largest contributors to greenhouse gas emissions in the world. In recent years, there has been an unprecedented increase in electricity demand driven by the so-called Artificial Intelligence (AI) revolution. Although AI has and will continue to have a transformative impact, its environmental and health impacts are often overlooked. The standard approach to power grid optimization aims to minimize CO$_2$ emissions. In this paper, we propose a new holistic paradigm. Our proposed optimization directly targets the minimization of adverse health outcomes under energy efficiency and emission constraints. We show the first example of an optimal fuel mix allocation problem aiming to minimize the average number of adverse health effects resulting from exposure to hazardous air pollutants with constraints on the average and marginal emissions. We argue that this new health-based power grid optimization is essential to promote truly sustainable technological advances that align both with global climate goals and public health priorities.

==> TCCML_NeurIPS_2024_Style_File/old_text.tex <==
%AI era 
Artificial Intelligence (AI) has rapidly emerged as a transformative technology with the potential to address some of the world's most pressing challenges. From revolutionizing agriculture with precision farming techniques[CITE] and crop health monitoring[CITE] to accelerating breakthroughs in cancer research through advanced predictive analytics[CITE], AI is heralded as a key driver of innovation and societal advancement. The deployment of AI systems promises substantial improvements in efficiency, accuracy, and scalability across various sectors, including climate change and health.
%AI driving up energy demand -> emissions -> health issues
However, amid the excitement surrounding AI's potential to solve critical issues, the environmental and health impacts associated with its deployment are often overlooked. The rapid proliferation of AI technologies demands vast computational resources, resulting in significant emissions of carbon dioxide (CO2) and hazardous air pollutants (HAP). These emissions stem from the substantial energy consumption required to power data centers, power-hungry facilities. The rise of Artificial Intelligence (AI) and the widespread adoption of generative AI models has profoundly impacted data centers' role, triggering an unprecedented surge in energy demand and new electricity consumption and exacerbating the strain on electricity resources and thus the existing challenges within the power grid infrastructure, and .[CITE]
The International Energy Agency (IEA) estimated that global data centers consumed between 240 to 340 terawatt-hours (TWh) in 2022,[CITE] accounting for approximately 1-1.3\% of global final electricity demand. This consumption is projected to double by 2026.
% bridge to power grid optimization including health
In this scenario, a key technical problem is the optimal allocation of resources, that allows for an efficient electrical, or power, grid optimization that ensure energy supply while keeping the environmental impacts under control.
%power grids
The electrical grid is a complex and interconnected system that ensures electric power delivery from energy producers to communities and industries around the world. As energy demand continues to grow, the need to optimize the grid has become increasingly pressing, involving the employment of advanced technologies and methods to enhance the efficiency of energy generation, transmission, and distribution, while also reducing costs and environmental impacts

